Mitigating Popularity Bias in Recommendation with Unbalanced Interactions: A Gradient Perspective

Recommender systems learn from historical user-item interactions to identify preferred items for target users. These observed interactions are usually unbalanced following a long-tailed distribution. Such long-tailed data lead to popularity bias to recommend popular but not personalized items to users. We present a gradient perspective to understand two negative impacts of popularity bias in recommendation model optimization: (i) the gradient direction of popular item embeddings is closer to that of positive interactions, and (ii) the magnitude of positive gradient for popular items are much greater than that of unpopular items. To address these issues, we propose a simple yet efficient framework to mitigate popularity bias from a gradient perspective. Specifically, we first normalize each user embedding and record accumulated gradients of users and items via popularity bias measures in model training. To address the popularity bias issues, we develop a gradient-based embedding adjustment approach used in model testing. This strategy is generic, model-agnostic, and can be seamlessly integrated into most existing recommender systems. Our extensive experiments on two classic recommendation models and four real-world datasets demonstrate the effectiveness of our method over state-of-the-art debiasing baselines.

==> Sections/Motivation_x.tex <==
\section{Problem Definition and Preliminaries}
In this section, we first formalize the definition of recommendation systems, for which the main goal is to infer personalized ranking of items based on user and item embeddings. Then we review Bayesian Personalized Ranking loss (BPR), and discuss what are the genuine factors that account for popularity bias in RS. Based on this, we propose a solution to mitigate such bias in an efficient and effective way.

\subsection {Problem Definition}
 Let $U = \{\boldsymbol{u_1}, \boldsymbol{u_2},,, \boldsymbol{u_N}\}$ and $I = \{\boldsymbol{i_1}, \boldsymbol{i_2},,,\boldsymbol{i_M}\}$ be the set of users and items, where $N$ and $M$ denote the number of users and items, respectively. We define the user-item interactions as $Y \in \{0,1\} ^{N \times M}$ where each $y_{ui}$  involves a user $u$ and item $i$ such that:
 \begin{equation}
 \begin{aligned}
  y_{ui}=\left\{\begin{matrix}
 1,& \quad \text{if  interaction between $u$ and $i$ is observed,}   \\ 
 0,& \quad \text{otherwise.}
\end{matrix}\right.
 \end{aligned}
 \end{equation}

We then denote the set of positive items for user $u$ as $I^+_u = \{i \in I | y_{ui} =1 \}$.

The goal of a recommender system is to learn a scoring function $f(u,i|\Theta)$ from the matrix $Y$, which is capable of predicting user preference over items with parameters $\Theta$. A typical matrix factorization (MF) recommender system model learns for each user and item a real-valued vector of latent features as model parameters. Let $boldsymbol{p_u} \in \mathbb{R}^D$ and $\boldsymbol{q_i} \in \mathbb{R}^D$ denote the latent vector for user $u$ and item $i$, respectively. MF estimates an interaction $\hat{y}_{ui}$ as the inner product of $\boldsymbol{p_u}$ and $\boldsymbol{\boldsymbol{q_i}}$ \cite{rendle2012bpr,he2017neural}:
\begin{equation}
    \hat{y}_{ui} = f(u,i|\boldsymbol{p_u},\boldsymbol{q_i}) = \sum_{d=1}^{D} p_{ud}\cdot q_{id} = \boldsymbol{p_u}^{T}\boldsymbol{q_i}.
\end{equation}

In the test phase, the RS task returns for a user $\boldsymbol{u}$ the personalized ranking $R_u$ of items in $I$ by ordering the items by:  
\begin{equation}
    score(u,i)  = \boldsymbol{p_u}^{T}\boldsymbol{q_i} =  \| \boldsymbol{q_i} \| cos(\boldsymbol{p_u},\boldsymbol{q_i}),
    \label{eq.ranking}
\end{equation}
where in the second equality $\| \boldsymbol{p_u} \|$ is omitted since it is invariant for a given user $u$.
%
In other words, the personalized ranking result during test stage only depends on the magnitude of  item embedding $\boldsymbol{q_i}$ and its cosine distance between the user embedding $\boldsymbol{p_u}$. In the training stage, we often adopt an objective function using the Bayesian Personalized Ranking (BPR) loss \cite{rendle2012bpr}. %or Binary Cross Entropy (BCE) loss \cite{} defined on the predicted $\hat{y}_{ui}$ and its ground truth $y_{ui}$ to train the model.
%
In the following, we shall revisit BPR loss functions for RS with implicit feedback. The analytical results shed light on the root cause that affects user and item embeddings and inspire us to design a simple yet effective solution in Section~\ref{sec:revisit}.

%Existing works mainly learn a unified representation to balance the distribution of popular and unpopular items. However, we still can not guarantee the relative value of $||i|| cos(u,i)$ . This motivations us the following two questions: 
%\begin{itemize}
%    \item What is the cause component for user and item embedding?
%    \item How such cause affect popularity bias? 
%\end{itemize}
%To further better answer the two questions, we first review the optimization process of two widely used Bayesian Personalized Loss (BPR) and Binary Cross Entropy loss (BCE) in recommendation system. 

%where $S(\dot)$ is a similarity function, e.g., dot production, which measure the ranking score $r_{ui}$ for user $u$ on an item $i$.
%In our scenario implicit feedback S ⊆ U×I is available.  Machine learning approaches for item recommenders [5, 10] typically create the training data from S by giving pairs (u, i) ∈ S a positive class label and all other combinations in (U × I) \ S a negative one (see Figure 1). Then a model is fitted to this data. That means the model is optimized to predict the value 1 for elements in S and 0 for the rest. The problem with this approach is that all elements the model should rank in the future ((U × I) \ S) are presented to the learning algorithm as negative feedback during training.
%To formalize this we create training data DS : U × I × I by:
\subsection{Revisit of BPR Loss}
\label{sec:revisit}
In realistic scenarios, only observations of positive implicit feedback (e.g., clicks and purchases) are available. The non-observed user-item pairs, e.g. a user has not purchased an item yet – are a mixture of real negative feedback (i.e., the user is not interested in the item) and missing values (i.e., the user has not seen the item which he or she is interested in)\cite{rendle2012bpr}. The training set is denoted by $D_s :=\{(u,i,j)|i\in I^+_u \wedge j \in (I\setminus I^+_u)\}$.

BPR loss is proposed based on the maximum posterior estimator for personalized item ranking:
% \textcolor{red}{if eq.4 is consistent with eq.2?}

\begin{equation}
    L_{BPR} = \sum_{(u,i,j)\in D_s }  \log \;(\sigma(\hat{y}_{ui}-\hat{y}_{uj}))-\lambda_\Theta ||\Theta||^2 ,
\end{equation}
where $\Theta$ is the model parameters and $\sigma(x) = \frac{1}{1+\exp(-x)}$ is the sigmoid function. %Formally, the problem of predicting $\hat(r_{ui})$ can be seen as the task of estimating a matrix $R : U \times I$. Thus, this prediction formula can be rewritten as:
%\begin{equation}
%    \hat{r_{ui}} = <w,h> = \sum_{f=1}^k w_{uf} \cdot h_{if} 
%\end{equation}
The gradient of BPR loss with respect to the model parameters $\Theta$ (e.g., user/item embeddings) can be written as:
\begin{equation}
\begin{aligned}
    \frac{\partial \; L_{BPR}}{\partial\; \Theta}&=\sum_{(u,i,j) \in D_S} \frac{\partial \, \log \sigma(\hat{y}_{ui}-\hat{y}_{uj}))}{\partial \, \Theta} - \lambda_{\Theta} 
\frac{\partial \, ||\Theta||^2}{\partial \, \Theta } \\
& \propto \frac{-e^{-(\hat{y}_{ui}-\hat{y}_{uj})}}{1+-e^{-(\hat{y}_{ui}-\hat{y}_{uj})}} \cdot \frac{\partial \,(\hat{y}_{ui}-\hat{y}_{uj})}{\partial \, \Theta} - \lambda_{\Theta} \Theta.
\end{aligned}
\end{equation}

%Considering the partially interaction records, \cite{} Personalized Bayesian Ranking (BPR) loss is proposed to model the ranking order than optimizing prediction loss on the whole item lists. \cite{}. 
More concretely, the gradients for updating a matrix factorization model are:
\begin{equation}
\frac{\partial \; (\hat{y}_{ui}-\hat{y}_{uj})}{\partial \; \Theta}
=
\left\{\begin{matrix}
 (q_{id}-q_{jd}) & \; \text{if} \; \Theta = p_{ud} \\
 p_{ud} & \; \text{if}  \; \Theta = q_{id}\\ 
 - p_{ud} & \; \text{if}  \; \Theta = q_{jd}\\ 
0 & \; \text{otherwise}.
\end{matrix}\right.
\end{equation}

For BPR loss optimization, we notice that for each user-item pair $(u,i)$ with positive interaction, the model will randomly sample a negative pair $(u,j)$. For a popular item $i$ which matches mainstream preference, it is frequently updated by a positive gradient $p_{ud}$ and by a negative gradient $-p_{ud}$ only when it served as a negative sample.
%
In other words, item $i$ will be updated with positive gradients more frequently than negative gradients during the optimization steps. The cumulative gradient update has a non-negligible impact on the optimized model, which can verified in Figure~\ref{Fig.main1}.

% {\color{blue} (EP: Need to say what impact. The figure on distribution of aggregated positive and negative gradient updates may fit very well here.)}
%Finally, even positive samples for category j might get a relatively low probability from the network.



==> Sections/supplementary_materials.tex <==
\section{supplementary}
\subsubsection{ \textbf{A revisit of BCE loss}}
Binary Cross-Entropy derives a multinomial distribution $p$ over each category from the model outputs $\hat{y}_{ui}$ in RS, and then computes the cross-entropy between the estimated distribution $p$ and ground truth distribution of $y_{ui}$. The Binary cross-entropy loss $L_{BCE}$ can be formulated as:
\begin{equation}
    L_{BCE} = \sum_{(u,i) \in D}  -y_{ui}\, \log(\hat{y}_{ui}) - (1-y_{ui})\:\log(1-\hat{y}_{ui})
\end{equation}

The derivative of the BCE loss with respect to the predicted interaction $\hat{y}_{ui}$ has the following formulation:
\begin{equation}
\begin{aligned}
\frac{\partial \; L_{BCE}}{\partial \; \hat{y}_{ui}}
=
\left\{\begin{matrix}
 p_j-1, & y_{ui} = 1\\
p_j, & y_{ui} = 0\end{matrix}\right.
\end{aligned}
\end{equation}

\textcolor{red}{
For the optimization of BCE, similar to BPR loss, we notice that for a popular item $i$ which often appears in observed interactions, it can also be taken as a negative sample for a non-observed interaction. So the non-observed interaction category $y=0$ will lead to a discouraging gradient $p_j$ for model updating, which further leads the RS model to predict low probability for the category $y=0$. If j is a rare category, the discouraging gradients will occur much more frequently than encouraging gradients 
in the iterations of optimization. The accumulated gradients will have a non-negligible impact on that category. Finally, even positive samples for category j might get a relatively low probability from the model.
}


==> Tables/different_loss.tex <==
\begin{table}[t]
\caption{Comparison between the proposed negative sampling strategy PNSM with traditional random strategy on Movielens-10M dataset.}
\centering
\vspace{-5px}
{\small
\begin{tabular}{lcccccc}
\toprule
&\multicolumn{3}{c}{Top-K=20}& \multicolumn{3}{c}{Top-K=50} \\
\cmidrule(r{1em}l{1em}){2-4}  \cmidrule(r{1em}l{1em}){5-7}
Name & Recall &  HR & NDCG & Recall &  HR & NDCG \\
\midrule
PNSM & \bf{0.1634} & \bf{0.5197} & \bf{0.1084} & \bf{0.2872} & \bf{0.6975} & \bf{0.1468} \\
RANDOM & 0.1274 & 0.4394 & 0.0843 & 0.2306 & 0.6255 & 0.1160 \\
\bottomrule
\end{tabular}\label{table:loss}
}
\vspace{-10px}
\end{table}

